Toward Multi-class Anomaly Detection: Exploring Class-aware Unified Model against Inter-class Interference

In the context of high usability in single-class anomaly detection models, recent academic research has become concerned about the more complex multi-class anomaly detection. Although several papers have designed unified models for this task, they often overlook the utility of class labels, a potent tool for mitigating inter-class interference. To address this issue, we introduce a Multi-class Implicit Neural representation Transformer for unified Anomaly Detection (MINT-AD), which leverages the fine-grained category information in the training stage. By learning the multi-class distributions, the model generates class-aware query embeddings for the transformer decoder, mitigating inter-class interference within the reconstruction model. Utilizing such an implicit neural representation network, MINT-AD can project category and position information into a feature embedding space, further supervised by classification and prior probability loss functions. Experimental results on multiple datasets demonstrate that MINT-AD outperforms existing unified training models.

==> CVPR/sec/0_abstract.tex <==
\begin{abstract}
Despite the rapid progress of unsupervised anomaly detection, most existing methods necessitate separate training processes for individual anomaly categories. 
Although several methods have strived to create unified models for multi-class anomaly detection tasks, they often overlook the utility of class labels, a potent tool for mitigating inter-class interference. 
To address this issue, we propose a \textit{Multi-class Implicit Neural representation Transformer for unified Anomaly Detection (MINT-AD)}, which leverages the fine-grained category information in the training stage. By learning the multi-class distributions, the model generates class-aware query embeddings for the transformer decoder, mitigating inter-class interference within the reconstruction model. Utilizing such an implicit neural representation network, MINT-AD can project category and position information into a feature embedding space, further supervised by classification and prior probability loss functions. Experimental results on multiple datasets demonstrate that MINT-AD outperforms existing unified training models. 
\end{abstract} 

==> CVPR/sec/1_intro.tex <==
\section{Introduction}
\label{sec:intro}
Recently, image anomaly detection (AD) and localization have been widely applied in the industrial quality inspection~\cite{cohen2020sub, yi2020patch,liu2023deep}, medical diagnosis~\cite{ding2022catching, salehi2021multiresolution}, and other fields. These applications aim to identify abnormal images and locate abnormal pixel regions. However, in real-world scenarios, only a small portion of data is abnormal, and the abnormal modality varies unpredictably, which hinders large-scale data collection and annotation. Therefore, most researches in this area are unsupervised~\cite{chen2022deep, qiu2022latent, li2022towards, jiang2022softpatch}, or supervised~\cite{li2021cutpaste, yao2022explicit} with artificial abnormal or generation techniques. 

% unified model的研究很重要， 但是挑战比较大
% While in practical usage, it may be necessary to sample different views of the same object to complete quality inspection better, and each view might require a separate model because of the appearance variations.
Among current State-Of-The-Art (SOTA) methods~\cite{liu2023simplenet, roth2021towards}, training a separate model for each class has shown high performance in current benchmarks. However, in practical applications such as industrial quality inspection, factories may prefer a single model to detect anomalies in multiple products or multiple views of a single object. Loading all models simultaneously into memory or frequently loading and unloading models during the AD process is not feasible due to the significant memory and time consumption. 
Therefore, a more practical approach is to train a single AD model for multiple object categories. However, training different categories together presents significant challenges due to inter-class interference, particularly in highly fragmented fields such as industrial inspection, where there are a massive number of subcategories of industrial products with differences and changes in various aspects. As shown in Figure~\ref{fig:toy-dataset}, we created a 2D toy dataset with a two-component Gaussian mixture and trained reconstruction models to get anomaly scores in the space. Ensembling two single-class models can obtain compact decision boundaries around normal distributions. When transferring a single-class model to a multi-class task, ``identical shortcut''~\cite{liu2023diversity} can be observed. However, a vanilla unified model cannot also obtain compact boundaries because neural networks tend to malfunction in complex inter-class regions, which is referred to as ``inter-class interference''. As a result, developing a unified anomaly detection model that can handle multiple object categories is a crucial but challenging task that requires innovative solutions. 

\begin{figure*}[tb]
    \centering
    \includegraphics[width=\linewidth]{CVPR/figures/figs-toy_dataset.pdf}
    \caption{Decision boundary on 2D synthetic multi-class data trained with different reconstruction-based anomaly detection methods. (a) Ensemble models training with two classes separately. (b) Single-class model trained with multi-class data, with ``identical shortcut'' happened broadly. (c) Vanilla unified model trained with all data simultaneously, where ``identical shortcut" around the two classes disappeared while ``inter-class interference'' appeared between two distributions. (d) Class-aware architecture in which class information leads to improved region boundaries.}
    \label{fig:toy-dataset}
\end{figure*}


% 当下的方法怎么解决的，还没解决好，
% TODO：还需要引入text embedding等方法，详细说明一下
% Although UniAD~\cite{you2022unified} has achieved the unification of anomaly detection models, they improved the robustness of the model by addressing the "identical shortcut" issue in the reconstruction model. 
% However, in reality, the "identical shortcut" issue also occurs in training models for a single class, but the complexity of the distribution in multi-class scenarios exacerbates this problem. 
Although existing multi-class AD models~\cite{you2022unified, Zhao_2023_CVPR, Lu2023HierarchicalVQ} has achieved the unification of anomaly detection models by addressing the ``identical shortcut" issue in the reconstruction model, they aim to capture the distribution of all classes simultaneously, allowing them to share the same boundary. For example, UniAD utilizes the same query embedding across multiple classes. However, this shared boundary may not exist, because the feature distribution differences between different classes are already significant. 
Rather than finding a common decision boundary for multi-class scenarios, reducing the interference between each class through category information is a simple and logical method for reconstructing anomalous features. 

% 我们是怎么解决多类之间的关系的
% we propose a multi-class anomaly detection model that utilizes category to assist in feature reconstruction based on the Transformer. Since the model is trained only on a training set containing normal samples, it can only reconstruct normal features well, and it have greater errors when reconstructing abnormal features. Based on this principle, the reconstruction-based model performs well in single-class anomaly detection, but multiple classes of data are input to the model for training, the model will confuse the reconstruction features of each due to the difficulty in distinguishing features of each class. To address this issue,

To mitigate the aforementioned issues, in this paper, we propose a novel MINT-AD method that uses an Implicit Neural Representation (INR) network to output the class-aware query of the reconstruction network. The class-aware query contains both the category information and the distribution of normal features of each category by two means: 
classification loss function to supervise the input of the perceptron to output a fine-grained category prompt;  
prior loss function to regularize feature adapter's outputs to Gaussian distributions and supervise the implicit neural representation network to predict the parameters of distributions. 
% Meanwhile, these two loss functions help regularize the adapted feature. 
Compared to previous research, this paper applies the multi-class anomaly detection setting to larger datasets. Experimental results show that MINT-AD outperforms existing unified training models and achieves consistent performance with the best single-class training model in most classes. 


% 我们设计了一个基于类别隐式编码的query embedding方式，来更好的减少类间干扰
% 我们用一个先验分布来更好的表述相关类别的每个像素的分布，来更好的完成特征重建
% 
\noindent We summarize our main contributions as follows:
\begin{itemize}
\item We find that ``inter-class interference'' is a problem of the unified AD model and class information can help to work it out. Then, we propose a novel approach that uses INR to utilize category information efficiently. 

\item We propose using fine-grained features from the classifier as prompts to provide more information on subclass distribution.

% \item The network learns class-aware queries by mapping the distribution of classes, which is a superior approach compared to other class-aware ways. And we have designed corresponding loss functions to provide supervision. 

\item Experimental results of both standard multi-class AD datasets and larger datasets demonstrate the effectiveness of the proposed method. 

% , which can significantly boost the performance of unified anomaly detection models and achieve state-of-the-art results on the MVTecAD benchmark. 
% \item We propose a novel approach (MINT) that can learn multi-class implicit neural representation for unified anomaly detection, improving both the accuracy and efficiency in real-world scenarios. 
%\item Redesigned transformer query embedding and compared different query compositions of category information, identifying an optimal approach for multi-class anomaly detection.
\end{itemize}

==> CVPR/sec/2_related_work.tex <==
% 当下的研究是什么，对应有什么缺点，我们怎么解决的？
\section{Related Work}

\subsection{Unsupervised Anomaly Detection}
% In natural data, acquiring anomalous data requires significant human resources as the majority of the data is normal, and only a small portion is anomalous. While some methods use synthesized defects~\cite{zavrtanik2021draem, li2021cutpaste, yao2022explicit} for training, it is difficult to simulate real defects and generalize all defects. In contrast, unsupervised methods only use normal data, treating all defects equally and eliminating the need for additional data synthesis processing, making them more robust. 
Recent research has focused on unsupervised methods~\cite{jiang2022survey}, which can be categorized into embedding-based~\cite{defard2021padim, roth2021towards} and reconstruction-based~\cite{bergmann2018improving, sabokrou2018adversarially, liu2020towards, chen2022utrad, you2022unified} methods. Embedding-based methods embed normal features into a compressed space, where anomalous features are far from the normal clusters in the embedding space. However, while embedding-based methods have achieved SOTA performance recently, computing the inverse or searching through the nearest neighbor in the memory bank limits real-time performance, especially for edge devices. Reconstruction-based methods, on the other hand, learn to reconstruct normal data and use the reconstruction error to identify anomalies. They do not require additional memory storage and have a simpler process. Our method is also based on reconstruction, but we directly perturb the features instead of augmenting the images at the image level to reconstruct the features.
% UniAD没有使用到类别信息，我们隐式的加入了
\subsection{Unified Model for Anomaly Detection}
Anomaly detection research has mainly focused on single-class scenarios, but UniAD~\cite{you2022unified} proposed the multi-class AD setting. UniAD addressed the "shortcut" problem by modifying the transformer network structure and proposing a hierarchical query decoder, a neighbor masking attention module, and a feature jittering strategy. 
Following this, OmniAL~\cite{Zhao_2023_CVPR} trains the unified model with proposed panel-guided synthetic anomaly data rather than directly using normal data and HVQ-Trans~\cite{Lu2023HierarchicalVQ} utilizes a hierarchical codebook mechanism to avoid shortcuts. 
However, while those methods enhanced the network structure for complex distributions, they didn't consider the uniqueness of multi-class tasks in terms of categories. 
% To address this, we propose using a classification network to implicitly embed class information, improving multi-class anomaly detection performance. 
To further enhance the performance of multi-class anomaly detection, we propose using implicit Neural Representation(INR)~\cite{park2019deepsdf,li2019grains, VincentSitzmann2020ImplicitNR, lindell2022bacon}. INR is a technique that represents object shape and appearance through function approximation without explicit mesh structures. This approach has been successfully applied in various fields, including computer vision, graphics, and robotics, but is novel for AD. 
% Inspired by SIREN~\cite{VincentSitzmann2020ImplicitNR}, we designed an implicit neural representation network composed of an MLP called the gated perceptron dual path. Additionally, we designed a prior distribution representation module with three multi-layer perceptrons to calculate the mean and variance of the distribution of features. This approach improves the representation and manipulation of objects' shape and appearance, making it a promising technique for multi-class anomaly detection.
%By adopting a classification network to implicitly embed class information and using INR to represent object shape and appearance, we can achieve more accurate and efficient anomaly detection in complex multi-class scenarios.

\begin{figure*}[ht]
    \centering
    \includegraphics[width=\linewidth]{CVPR/figures/query.pdf}
    \caption{\textbf{Class-aware Architecture Improvement}. (a) The vanilla UniAD~\cite{you2022unified} has a shared query for all categories in each layer of the decoder. We propose three approaches to enhance the structure for accommodating class prompts: (b) One simple way is using different queries for different classes. (c) Concatenating the class token before the image feature is intuitive. (d) Using a network to map the prompt into a query can also incorporate category information. }
    \label{fig:class_embed}
\end{figure*}

\subsection{Class-aware Networks}
% The Transformer~\cite{vaswani2017attention} model, originally designed for natural language processing, has been successfully applied in various computer vision tasks, such as detection, classification, and place localization. Most of the existing approaches use learnable queries that are randomly initialized~\cite{carion2020end}, while some researchers have explored how to design queries to improve performance. % that uses category priors represented by an external object detection model. However, CATN only uses category text information and a word2vector model to obtain the category text embedding vector. 
Networks can utilize category information to enhance performance in many aspects. For instance, CATN~\cite{dong2022category} is a transformer-based HOI model that uses category text information to initialize the object query. 
MCTformer~\cite{xu2022multi} proposes using multiple class queries within the transformer to capture class-specific attention, resulting in more discriminative object localization. 
% MCTformer~\cite{xu2022multi} proposes using multiple class queries. By learning multiple class tokens within the transformer, these queries can effectively capture class-specific attention, resulting in more discriminative object localization. 
CQL~\cite{xie2023category} proposes a query that is strongly associated with interaction categories. 
% In addition to the explicit query design, CQL~\cite{xie2023category} proposes a query that is strongly associated with interaction categories, which is converted to an image-specific category representation via a transformer decoder and learned through an auxiliary image-level classification task. 
However, these methods utilize category information that is associated with the supervised task. MaxQuery~\cite{yuan2023devil} proposes to use cluster centers of object queries in mask transformers. It can be applied to medical OOD tasks since the model has already recognized and clustered a limited number of object categories. 
% Drawing inspiration from the aforementioned methods, we developed a novel approach that utilizes a category-related implicit expression query. Unlike other methods, our approach does not require the use of an additional text-encoder pre-training network or multiple queries. Instead, we input the image information directly into a classification network and use the corresponding score vector obtained after implicit neural representation to generate the query.


%TODO：添加类别提示的方法

% In addition to traditional computer vision applications, researchers have also explored the use of Transformer for anomaly detection~\cite{mishra2021vt, pirnay2022inpainting, lee2022anovit, you2022unified}. InTra~\cite{pirnay2022inpainting}, VT-ADL~\cite{mishra2021vt}, and AnoVit~\cite{lee2022anovit} directly utilize vanilla Transformer, without investigating why Transformer brings improvement. UniAD~\cite{you2022unified} designed a layer-wise query decoder to confirm the efficacy of the query embedding to prevent shortcut. To address these issues, we propose an image-based feature embedding queries for the Transformer decoder network. This approach aims to improve the performance of anomaly detection by leveraging image features to design more effective queries.

==> CVPR/sec/3_methods.tex <==
\section{Methods}

% In this section, we present a comprehensive introduction to our proposed MINT-AD. As depicted in Figure\ref{fig:MINT}, MINT-AD comprises a basic feature extractor, a category classifier and encoder, and a reconstruction network. We will provide a detailed description of each corresponding module in the following sections. 



% 说明类别信息很重要，如何把类别进行引入进去，后面的章节则是详细阐述
\subsection{Class-aware Improvement}
As shown in Figure~\ref{fig:class_embed}, traditional unified networks cannot directly receive and utilize class information, but we can achieve class prompting by modifying the network structure. One approach is to establish a query pool, where different classes use different queries during the reconstruction process to address the interference caused by shared queries. However, this approach has limited scalability. Another more direct approach is to generate a class token, which delegates the task of distinguishing between classes to the self-attention mechanism implicitly. Utilizing prompt mapping with cross-attention is a more flexible solution. For example, we can construct class-related text and use existing text encoders to extract and integrate class information. Existing work has shown that both images ~\cite{chen2021crossvit} and text ~\cite{rombach2022high} can serve as such prompts. 
So, we further explore the type of prompt and the structure for mapping.
\subsection{Overview of Model}
\label{adapter}
We introduce MINT-AD, a novel unified anomaly detection and reconstruction model based on the Transformer framework, which leverages class-specific object-aware reconstruction. The overall architecture of MINT-AD is illustrated in Figure \ref{fig:MINT}. 
The main reconstruction network is a transformer with a 6-layer encoder and decoder. We use INR to output the class-aware query and a distribution decoder to predict the distribution parameters of the adapted image feature. Using INR in anomaly detection tasks is innovative, and we believe it is a better way to incorporate class information. 
% After passing through the classification network, we embed the features with positional information and input them into the implicit encoding network to learn a class-specific query, which forms the input query of the Transformer decoder. To better utilize class information, we design a prior distribution decoder to estimate the mean and variance of corresponding class pixels. This helps to regular the feature distribution and supervise the query. 

% However, the interference between multiple classes remains unpredictable due to the shared query embedding. Alternatively, one can use multiple queries indexed by class or utilize a text encoder. However, these methods require class information during testing, and through comparative experiments, we have demonstrated the effectiveness of queries from class-prompted mapping. 
\begin{figure*}[htb]
    \centering
    \includegraphics[width=0.9\linewidth]{CVPR/figures/network.pdf}
    \caption{\textbf{Architecture of MINT-AD network}. 1. A dual-path INR network with different activation functions is introduced to map position encoding and class-aware prompt to the image feature dimension and assist the reconstruction transformer through cross-attention as queries. 2. We are trying to find a fine-grained prompt that can map the distribution of subcategories. 3. Therefore, we do not directly generate prompts from the (a) image or (b) label but extract (c) subcategory features from the classification network from the image to label as the prompt. 
    % The main structure of the MINT-AD network omits the feature extraction part using a pre-trained network. MINT-AD is mainly divided into two parts, where the gray part (a)(d) is the basic reconstruction network, and the blue part (b)(c) is the multi-class implicit neural representation network, which is further divided into two blocks. The left block is the category-supervised implicit neural representation module, and the right block is the prior distribution module.
    }
    \label{fig:MINT}
\end{figure*}

During training, we follow UniAD to simulate real-world scenarios and extract class information using a pre-trained EfficientNet~\cite{tan2019efficientnet} as the feature extractor, which is frozen during training. As our training data only contains normal samples, we add Gaussian perturbations to the features to enhance the representation and reconstruction capabilities of normal classes. However, pre-trained feature extractors may not be optimal for anomaly detection data, as pointed out by some anomaly detection research ~\cite{liu2023simplenet,zou2022spot,Reiss2021PANDAAP}. Therefore, we employ a feature adaptor (a single fully connected layer by default) to transform the features into a specific domain. We denote the original image feature as $\boldsymbol{f'}$ and the adapted feature as $\boldsymbol{f}$, while the single patch feature among them is represented by $\phi '$ and $\phi$, respectively.

% Before being processed by the reconstruction network, the image input undergoes feature extraction via a pre-trained feature extractor, and the parameters of this pre-trained network are frozen during the training process. Following UniAD, we use EfficientNet-b4~\cite{tan2019efficientnet} pre-trained on ImageNet~\cite{deng2009imagenet} as the feature extractor and extract features from different intermediate layers, which are scaled to the same size and concatenated to form the feature.
% After that, a perturbation is sampled from the Gaussian distribution and directly added to form the perturbed feature. This operation guides the model to learn the knowledge of normal samples through denoising tasks while enhancing the robustness of the classification and reconstruction network. As highlighted in previous anomaly detection studies ~\cite{liu2023simplenet,zou2022spot,Reiss2021PANDAAP}, pre-trained feature extractors may be suboptimal for anomaly detection data. We employ a feature adaptor (defaulting to a single fully connected layer) to transform the features to a specific domain. We notate the unperturbed feature as $\boldsymbol{f'}$ and the adapted feature as $\boldsymbol{f}$, while the single patch feature among them is represented by $\phi '$ and $\phi$, respectively.  

% $\mathcal{D}= \{\boldsymbol{f}_i\}_i^|\mathcal{D}|$ notates the training feature set and $\phi = \boldsymbol{f}_{hw} \in \mathbb{R}^{C}$ is a feature in the feature map. 

% After obtaining the parameters corresponding to the input sample image, a perturbation matching its size is generated and directly added to form the perturbed feature. This operation guides the model to learn the knowledge of normal samples through denoising tasks while enhancing the robustness of the classification network. Specifically, we sample noise from a Gaussian distribution with a scale related to the original feature scale. Let $\boldsymbol{f}\in \mathbb{R}^{C\times H\times W}$ represents the extracted feature, and $\phi = \boldsymbol{f}_{hw} \in \mathbb{R}^{C}$ is a feature in the feature map. The jitter is a sampling from Gaussian distribution $D \sim N\left(\mu=0, \sigma=\left(\alpha {\left\|\boldsymbol{f}\right\|_2}/{C}\right)\right)$, where $\alpha$ is a hyperparameter that controls the size of the perturbation. Note that the perturbation is only added during the training phase, and no perturbation is added during the testing phase to ensure the best reconstruction performance. As pointed out by some AD research ~\cite{liu2023simplenet,zou2022spot,Reiss2021PANDAAP}, pre-trained feature extractors may be suboptimal for anomaly detection data. Therefore, we employ a feature adaptor (a single fully connected layer by default) to transform the features into a specific domain. The adapted feature is notated by $\boldsymbol{f}'$. 


% \begin{equation}
% D \sim N\left(\mu=0, \sigma^2=\left(\alpha \frac{\left\|\boldsymbol{f}\right\|_2}{C}\right)^2\right),
% \end{equation}


%The perturbed feature $\boldsymbol{f}'\in \mathbb{R}^C$C is then input into the basic reconstruction network and the multi-category implicit representation network. The basic reconstruction network is a multi-layer network based on the Transformer structure, which uses the same neighbor masking attention module as UniAD, and the output of the implicit representation network is used as the query for each layer of the decoder.

\subsection{Class-aware Implicit Neural Representation}
\label{INR}
To ensure that the reconstruction model can distinguish between multiple categories of data and that the reconstruction of each category is not affected by other categories, this paper proposes using different query values for different categories to make the reconstruction process robust to multiple categories.

\noindent\textbf{Classfication Representation}. Since we cannot guarantee that each data sample has a category label, a classifier is used to predict the category of each sample. The classifier uses adapted feature $\boldsymbol{f}$ as input. After passing through the category encoder $E_{class}$ and the classification head, it obtains the predicted value $\hat{y}=head(E_{class}(\boldsymbol{f}))\in \mathbb{R}^{N}$, which is then used to calculate the cross-entropy loss with the one-hot encoded category label $y \in \mathbb{R}^{N}$ as shown in Equation~\ref{eq:celoss}:
\begin{equation}\label{eq:celoss}
    \mathcal{L}_{CE}=-\frac{1}{N}\sum_{c=0}^{N-1} y_{c} \log \hat{y}_{c}. 
\end{equation}
\noindent\textbf{Implicit Neural Representation}. 
However, we found that the granularity of category labels in industrial anomaly detection is not fine enough. For example, in MVTec AD dataset, the ``toothbrush" category includes various colors, and the ``screw" category has multiple placement postures. Therefore, we propose to use finer-grained classification features as prompts for the unified model. 
% To address the issue of subcategories caused by differences in the distribution of data within a single category due to factors such as changes in the position of the photographed object, rotation of the shooting angle, and domain shift of the object itself, 
As shown in Figure 3, this paper does not directly use the predicted category label or image feature, but instead uses the token $t_{c} = E_{class}(\boldsymbol{f}) \in \mathbb{R}^{N'}$ before the last classification head as the representation of the subcategory. The key issue addressed in this section is mapping from low-dimensional logistic regression to high-dimensional queries. 
We propose that Multi-Layer Perceptron (MLP) is inefficient, which requires a massive number of parameters to accomplish this high-dimensional mapping. Implicit neural representation~\cite{mildenhall2021nerf}, on the other hand, is well-suited for solving this high-dimensional mapping problem from discrete values to continuous values. INR is a continuous function mapping position encoding to values, and to enable it to map different categories, we use the idea from the concept of multiple instances Neural Radiance Fields and employ a dual-path structure. Like the position encoding in Transformer, the position encoding uses a learnable embedding. 

Similar to~\cite{mehta2021modulated}, the dual-path structures use different activation functions to achieve different functions. The MLP that takes the position encoding as input is called the synthesis network, which implements the mapping from coordinates to signal values and uses sine functions as activation functions, like SIREN~\cite{VincentSitzmann2020ImplicitNR}. The MLP that takes the category encoding as input is called the modulator, which uses a ReLU-based function activation. The modulator is the key to category generalization, and it outputs the amplitude, phase, and frequency parameters of the periodic activation in the modulated synthesis network at each layer. 

Implicit neural networks can effectively map category information to the feature dimension. However, we expect the corresponding feature space to be continuous. Additionally, class token $t_c$ should correspond to the entire subclass of samples rather than individual instances. Therefore, we further design prior distribution representation and prior loss functions to supervise the mapping process. 

% \begin{figure*}[htb]
%     \centering
%     \includegraphics[width=\linewidth]{NeurIPS/figures/feature_embedding_all_crop.pdf}
%     \caption{\textbf{Class embedding methods schematic diagram}. The blue variable "z" represents the class label.(a) The label is simply concatenated with the feature vector; (b) The label is used to select a query from a pool of multiple queries; (c) The label is used to supervise the learning of class-aware query embeddings.}
%     \label{fig:class_embed}
% \end{figure*}


% \begin{figure}[t] 
% \centering
% \subfigure[Label embedding]{
% 	\begin{minipage}[b]{0.3\textwidth}
% 		\includegraphics[width=1\textwidth]{NeurIPS/figures/class_embedding/class_embedding_full_crop_1-1.pdf}
% 	\end{minipage}
% 	\label{fig:label_embedding}
%     } \hspace{0.1cm}
% \subfigure[Multiple query pool embedding]{
%     \begin{minipage}[b]{0.3\textwidth}
%     \includegraphics[width=1\textwidth]{NeurIPS/figures/class_embedding/class_embedding_full_crop_2-2.pdf}
%     \end{minipage}
%     \label{fig:multiple_query}
% }\hspace{0.1cm}
% \subfigure[Class-aware query embedding]{
%     \begin{minipage}[b]{0.3\textwidth}
%     \includegraphics[width=1\textwidth]{NeurIPS/figures/class_embedding/class_embedding_full_crop_4-end.pdf}
%     \end{minipage}
%     \label{fig:class_aware_embedding}
% }
% \caption{\textbf{Class embedding methods schematic diagram}. The blue variable "z" represents the class label. (a) The label is concatenated with the feature vector; (b) The label is used to select a query from a pool of multiple queries; (c) The label is used to supervise the mapping of class-aware query while the "x" represents coordinate.}
% \label{fig:class_embed}
% \end{figure}

\subsection{Prior Distribution Representation}
% 如何设计prior loss的，以及理论基础
% The prior distribution representation module contains three multi-layer perceptrons, where the implicit neural representation network is composed of an MLP called the gated perceptron dual path, and the output representation is mapped to the mean and variance of the distribution of the features through an MLP as the distribution decoder. 
% Since each category label corresponds not to a single image or object but to the distribution of all normal samples in that category, the image features are not directly used to supervise the output of the gated perceptron. Instead, they are mapped to a prior distribution and supervised using the posterior probability of each sample. 

Since each subclass represents a distribution of normal images, we introduce an additional decoder to map the features output by INR into parameters for Gaussian distributions of image features. 
% \paragraph{Lemma 1.} 
Assuming that all image features within the same subclass $\{\boldsymbol{f'}_c\}$ can be projected onto the same token $t_{c}$, we can use a predefined distribution $q(\omega_c)$ to estimate the statistics of features, where the parameters $\omega_c$ of this distribution can be derived from class token mappings. 
Since we use neural networks to get $w_c$. The parameters of whole distribution networks $\theta_p$ are estimated with maximum likelihood estimation:
\begin{equation}
{\theta_p}^*=\arg \max _{\theta_p} \frac{1}{|\mathcal{D}|} \sum_{\boldsymbol{f} \in \mathcal{D}} \log \mathcal{P}_{\theta_p}\left( \boldsymbol{f'}_c \mid q(\omega_c)\right).
\end{equation}
% The parameter $\theta$ represents the combined parameters of the feature adapter $\theta_a$ and the representation module $\theta_p$
% With parameters of feature adapter $\theta_a$ and parameters of representation module $\theta_p$, 
However, the distribution functions for different categories may vary. To standardize the distribution of image features, we propose using a network to adapt the image features. We reuse the adapter mentioned in Section \ref{adapter} to transform the estimation of original image features into an estimation of adapted feature distribution. 
The log-likelihood can be rewritten as
\begin{equation}
\begin{split}
\log \mathcal{P}_{\{\theta_p, \theta_a\}}( \boldsymbol{f}_c \mid & q(\omega_c))  = \mathcal{L}_{E L B O}(q, \theta_a) \\
&+ KL[q(\omega_c \mid t_{c},\theta_p) \| p_{\theta_a}(\boldsymbol{f'}_c)], 
\end{split}
\end{equation}
where $\theta_a$ is parameter of adapter, and $q(\omega_c)$ try to approximate the adapted feature distribution $\mathcal{P}_{\theta_a}(\boldsymbol{f'}_c)$. The feature adaptor optimizes the evidence lower bound $\mathcal{L}_{E L B O}$, and distribution projection optimizes the Kullback-Leibler divergence $KL[.]$. So, these two modules can be optimized by a single prior loss function. 
The preset distribution $q$ for the entire image features can be set as the joint distribution of distributions for each position. 
Ignoring the conditional dependence, we set the distribution in each position as an independent normal distribution. 
The decoder that maps the distribution only needs to output the mean $\mu$ and variance $\sigma$ for each position. The prior loss can be defined as 
\begin{equation}\label{eq:priorloss}
    \mathcal{L}_{Prior}=\sum_{\phi \in \boldsymbol{f}} -\log \mathcal{P}(\phi | \mathcal{N}(\mu,\sigma)).
\end{equation}


% \subsection{Query Embedding Transformer for Reconstruction}
% We use a basic reconstruction network composed of 4 layers of Transformer encoders and 4 layers of Transformer decoders. Except for the attention module, the other parts of the network are consistent with the basic structure of Transformer~\cite{vaswani2017attention}. Let $E^l$ denote the input of each layer of the Transformer encoder, where $l$ is the corresponding layer number, and let $E^{l+1}$ denote the output of that layer, since each layer is connected. The input of each layer of the Transformer decoder is denoted by $D^l$. The attention module of the encoder can be represented as
% \begin{equation}
% \operatorname{Attn}e\left(E^l\right)=\operatorname{Softmax}\left[\operatorname{Mask}\left(\frac{\left(E^l W_Q^l\right)\left(E^l W{\mathcal{K}}^l\right)^{\prime}}{\sqrt{d}}\right)\right]\left(E^l W_{\mathcal{V}}^l\right),
% \end{equation}
% where $W_Q^l,W_K^l,W_V^l$ are learnable parameter matrices used to generate queries, keys, and values (Q, K, V), and $d$ is the dimension of all three. The input of the first layer encoder is the perturbed feature $E^0=\boldsymbol{f}'$. $Mask()$ is the neighbor masking module used in UniAD, which masks the diagonal elements representing itself and the surrounding pixels to $-\infty$ and adds them to the output.

% We utilized a basic reconstruction network consisting of 4 layers of Transformer encoders and 4 layers of Transformer decoders. Unlike traditional query embedding methods that use a single learnable initialized query, we designed an implicit class representation query embedding method. Each layer of the Transformer decoder contains two attention layers. The first attention layer uses the output of the last layer of the encoder $E^{L+1}$ mapped to keys and values, and the output of the implicit representation network $\boldsymbol{q}$ as the query:
% \begin{equation}
% \operatorname{Attn}{d1}\left(E^{L+1},\boldsymbol{q}\right)=\operatorname{Softmax}\left[\operatorname{Mask}\left(\frac{\boldsymbol{q}\left(E^{L+1} W{\mathcal{K}}^l\right)^{\prime}}{\sqrt{d}}\right)\right]\left(E^{L+1} W_{\mathcal{V}}^l\right).
% \end{equation}
% The second attention layer uses the sum of the output of the first layer and $\boldsymbol{q}$ as the new query, and maps the output of the previous layer of the decoder to keys and values:
% \begin{equation}
% \operatorname{Attn}{d2}\left(D^l,\boldsymbol{q}\right)=\operatorname{Softmax}\left[\operatorname{Mask}\left(\frac{(\operatorname{Attn}{d1}\left(E^{L+1},\boldsymbol{q}\right)+\boldsymbol{q})\left(D^l W_{\mathcal{K}}^l\right)^{\prime}}{\sqrt{d}}\right)\right]\left(D^l W_{\mathcal{V}}^l\right).
% \end{equation}
% The input of the first layer decoder is the output of the last layer encoder $D^0=E^{L+1}$.

% The Euclidean distance between the final output of the basic reconstruction network and the original unperturbed feature is the reconstruction loss, and the reconstructed feature is denoted as 
% $\hat{\boldsymbol{f}}\in \mathbb{R}^{C\times H\times W}, \hat{\phi} = \hat{\boldsymbol{f}}_{hw} \in \mathbb{R}^{C}$. We use the mean squared error (MSE) loss function:
% \begin{equation}\label{eq:mseloss}
% \mathcal{L}_{MSE}=\frac{1}{H \times W} |\boldsymbol{f}- \hat{\boldsymbol{f}}|^2_2.
% \end{equation}

% \begin{figure*}[htp]
% \centering
% % \includegraphics[width=0.96\textwidth]{imgs/visualization.png}
% \resizebox{.96\textwidth}{!}{
%     \begin{tabular}{@{}cc@{}}
%         \multicolumn{1}{c}{\includegraphics[]{NeurIPS/figures/embedding1.png}} & 
%         \multicolumn{1}{c}{\includegraphics[]{NeurIPS/figures/embedding2.png}}
%     \end{tabular}
% }
% \caption{\textbf{Class embedding methods.} }
% \label{fig5}
% \end{figure*}
\subsection{Loss Function}
The output mapped by INR from fine-grained category features will serve as the query for the reconstruction network and interact with the image features in the cross-attention of each decoder layer. With the introduction of category information, the reconstruction network can reduce interference between categories. We maintain the mean squared error (MSE) loss function as the reconstruction supervisor: 
\begin{equation}\label{eq:mseloss}
\mathcal{L}_{MSE}=\frac{1}{H \times W} |\boldsymbol{f'}- \hat{\boldsymbol{f}}|^2_2,
\end{equation}
where $\hat{\boldsymbol{f}}$ is the reconstructed feature. 

The overall loss function is shown in Equation~\ref{eq:total_loss}, where $\lambda_a$ and $\lambda_b$ are weighting coefficients, which are set to 1 and 0.1, respectively, to optimize the classification and reconstruction networks first, as classification accuracy is a prerequisite for isolating reconstruction of each category, and the Transformer reconstruction network is more difficult to optimize.
\begin{equation}\label{eq:total_loss}
    \mathcal{L}_{total}= \mathcal{L}_{MSE} + \lambda_a \mathcal{L}_{CE} + \lambda_b \mathcal{L}_{Prior} .
\end{equation}

% \subsection{Convergence Analysis}

\subsection{Inference and Anomaly Score Function}
During the testing phase, except for not adding perturbations, all other parts of the network remain unchanged. Since the prior loss is a relatively fuzzy mapping, the reconstruction error is directly used as the anomaly score. For anomaly localization, the anomaly image is composed of the reconstruction distance of the feature map and is linearly interpolated to the size of the image input. The anomaly score of each patch feature before interpolation is:
\begin{equation}
s_{hw} = |\phi '- \hat{\phi}|^2_2 .
\end{equation}
For anomaly detection, the image-level anomaly score is the maximum value of the pixel-level anomaly score, which is generated by linearly interpolating the anomaly map of the feature dimension.
% i.e., taking the maximum value of the feature dimension:
% \begin{equation}
% S =\max {s_{hw}|h=1,...,H, w=1,...,W}.
% \end{equation}

==> CVPR/sec/4_experiments.tex <==
% 补充可视化结果
\begin{figure*}[htb]
    \centering
    \includegraphics[width=0.06\textwidth]{NeurIPS/figures/mvtec_viz/carpet.pdf}
    \includegraphics[width=0.06\textwidth]{NeurIPS/figures/mvtec_viz/grid.pdf}
    \includegraphics[width=0.06\textwidth]{NeurIPS/figures/mvtec_viz/leather.pdf}
    \includegraphics[width=0.06\textwidth]{NeurIPS/figures/mvtec_viz/zipper.pdf}
    \includegraphics[width=0.06\textwidth]{NeurIPS/figures/mvtec_viz/wood.pdf}
    \includegraphics[width=0.06\textwidth]{NeurIPS/figures/mvtec_viz/tile.pdf}
    \includegraphics[width=0.06\textwidth]{NeurIPS/figures/mvtec_viz/bottle.pdf} 
    \includegraphics[width=0.06\textwidth]{NeurIPS/figures/mvtec_viz/cable.pdf}
    \includegraphics[width=0.06\textwidth]{NeurIPS/figures/mvtec_viz/capsule.pdf}
    \includegraphics[width=0.06\textwidth]{NeurIPS/figures/mvtec_viz/metal_nut.pdf}
    \includegraphics[width=0.06\textwidth]{NeurIPS/figures/mvtec_viz/hazelnut.pdf}
    \includegraphics[width=0.06\textwidth]{NeurIPS/figures/mvtec_viz/transistor.pdf}
    \includegraphics[width=0.06\textwidth]{NeurIPS/figures/mvtec_viz/toothbrush.pdf}
    \includegraphics[width=0.06\textwidth]{NeurIPS/figures/mvtec_viz/screw.pdf}
    \includegraphics[width=0.06\textwidth]{NeurIPS/figures/mvtec_viz/pill.pdf}\\
    \caption{Qualitative results, where sampled image, ground truth, and anomaly map are shown for each class in MVTec AD.}
    \label{mvtec_figure}
\end{figure*}


\begin{table*}[ht]
\centering
\setlength\tabcolsep{3pt}
\caption{Performance comparison of different methods in anomaly detection with MVTec AD. (Metrics: I-AUROC of Unified/\textcolor{lightgray}{Separate})}
\resizebox{0.9\linewidth}{!}{
\begin{tabular}{ll|ccccccc}
\toprule\toprule
\multicolumn{2}{c|}{Categories} & PaDiM~\cite{defard2021padim} & CutPaste~\cite{li2021cutpaste} & DRAEM~\cite{7} & SimpleNet~\cite{liu2023simplenet} & UniAD~\cite{you2022unified} & OmniAL~\cite{Zhao_2023_CVPR} & MINT-AD(ours) \\ \midrule
\multirow{10}{*}{\rotatebox{90}{Objects}} 
&Bottle & 0.979/\textcolor{lightgray}{0.992} & 0.679/\textcolor{lightgray}{0.982} & 0.946/\textcolor{lightgray}{0.991} & 0.908/\textcolor{lightgray}{1.000} & 0.997/\textcolor{lightgray}{1.000} & \textbf{1.000}/\textcolor{lightgray}{0.994} & \textbf{1.000}/\textcolor{lightgray}{0.992} \\
&Cable & 0.709/\textcolor{lightgray}{0.971} & 0.692/\textcolor{lightgray}{0.812} & 0.618/\textcolor{lightgray}{0.947} & 0.561/\textcolor{lightgray}{0.999} & 0.952/\textcolor{lightgray}{0.976} & \textbf{0.982}/\textcolor{lightgray}{0.976} & 0.935/\textcolor{lightgray}{0.986} \\
&Capsule & 0.734/\textcolor{lightgray}{0.875} & 0.630/\textcolor{lightgray}{0.982} & 0.702/\textcolor{lightgray}{0.985} & 0.777/\textcolor{lightgray}{0.974} & 0.869/\textcolor{lightgray}{0.853} & 0.952/\textcolor{lightgray}{0.924} & \textbf{0.955}/\textcolor{lightgray}{0.810} \\
&Hazelnut & 0.855/\textcolor{lightgray}{0.994} & 0.809/\textcolor{lightgray}{0.983} & 0.951/\textcolor{lightgray}{1.000} & 0.820/\textcolor{lightgray}{1.000} & 0.998/\textcolor{lightgray}{0.999} & 0.956/\textcolor{lightgray}{0.980} & \textbf{1.000}/\textcolor{lightgray}{1.000} \\
&Metal nut & 0.880/\textcolor{lightgray}{0.962} & 0.600/\textcolor{lightgray}{0.999} & 0.889/\textcolor{lightgray}{0.987} & 0.501/\textcolor{lightgray}{1.000} & \textbf{0.992}/\textcolor{lightgray}{0.990} & 0.992/\textcolor{lightgray}{0.999} & \textbf{0.993}/\textcolor{lightgray}{0.971} \\
&Pill & 0.688/\textcolor{lightgray}{0.901} & 0.714/\textcolor{lightgray}{0.949} & 0.690/\textcolor{lightgray}{0.989} & 0.595/\textcolor{lightgray}{0.990} & 0.937/\textcolor{lightgray}{0.883} & \textbf{0.972}/\textcolor{lightgray}{0.977} & 0.958/\textcolor{lightgray}{0.983} \\
&Screw & 0.569/\textcolor{lightgray}{0.975} & 0.852/\textcolor{lightgray}{0.887} & 0.933/\textcolor{lightgray}{0.939} & 0.486/\textcolor{lightgray}{0.981} & 0.875/\textcolor{lightgray}{0.919} & 0.880/\textcolor{lightgray}{0.810} & \textbf{0.983}/\textcolor{lightgray}{0.978} \\
&Toothbrush & 0.953/\textcolor{lightgray}{1.000} & 0.639/\textcolor{lightgray}{0.994} & 0.828/\textcolor{lightgray}{1.000} & 0.608/\textcolor{lightgray}{0.997} & 0.942/\textcolor{lightgray}{0.950} & \textbf{1.000}/\textcolor{lightgray}{1.000} & \textbf{1.000}/\textcolor{lightgray}{0.956} \\
&Transistor & 0.866/\textcolor{lightgray}{0.944} & 0.579/\textcolor{lightgray}{0.961} & 0.839/\textcolor{lightgray}{0.931} & 0.678/\textcolor{lightgray}{1.000} & \textbf{0.998}/\textcolor{lightgray}{1.000} & 0.938/\textcolor{lightgray}{0.938} & \textbf{0.998}/\textcolor{lightgray}{0.999} \\ \midrule
&Zipper & 0.797/\textcolor{lightgray}{0.986} & 0.935/\textcolor{lightgray}{0.999} & 0.991/\textcolor{lightgray}{1.000} & 0.837/\textcolor{lightgray}{0.999} & 0.958/\textcolor{lightgray}{0.967} & \textbf{1.000}/\textcolor{lightgray}{1.000} & 0.991/\textcolor{lightgray}{0.996} \\
\multirow{5}{*}{\rotatebox{90}{Textures}}  
&Carpet & 0.938/\textcolor{lightgray}{0.998} & 0.936/\textcolor{lightgray}{0.939} & 0.959/\textcolor{lightgray}{0.955} & 0.902/\textcolor{lightgray}{0.997} & 0.998/\textcolor{lightgray}{0.999} & 0.987/\textcolor{lightgray}{0.996} & \textbf{0.999}/\textcolor{lightgray}{1.000} \\
&Grid & 0.739/\textcolor{lightgray}{0.967} & 0.932/\textcolor{lightgray}{1.000} & 0.981/\textcolor{lightgray}{0.999} & 0.609/\textcolor{lightgray}{0.997} & 0.982/\textcolor{lightgray}{0.985} & 0.999/\textcolor{lightgray}{1.000} & \textbf{1.000}/\textcolor{lightgray}{0.999} \\
&Leather & 0.999/\textcolor{lightgray}{1.000} & 0.934/\textcolor{lightgray}{1.000} & 0.999/\textcolor{lightgray}{1.000} & 0.859/\textcolor{lightgray}{1.000} & \textbf{1.000}/\textcolor{lightgray}{1.000} & 0.990/\textcolor{lightgray}{0.976} & \textbf{1.000}/\textcolor{lightgray}{1.000} \\
&Tile & 0.933/\textcolor{lightgray}{0.981} & 0.886/\textcolor{lightgray}{0.946} & 0.983/\textcolor{lightgray}{0.996} & 0.902/\textcolor{lightgray}{0.998} & 0.993/\textcolor{lightgray}{0.990} & \textbf{0.996}/\textcolor{lightgray}{1.000} & 0.992/\textcolor{lightgray}{0.990} \\
&Wood & 0.721/\textcolor{lightgray}{0.992} & 0.804/\textcolor{lightgray}{0.991} & \textbf{0.998}/\textcolor{lightgray}{0.991} & 0.907/\textcolor{lightgray}{1.000} & 0.986/\textcolor{lightgray}{0.979} & 0.932/\textcolor{lightgray}{0.987} & 0.994/\textcolor{lightgray}{0.989} \\ \midrule
&\textbf{Mean} & 0.842/\textcolor{lightgray}{0.958} & 0.775/\textcolor{lightgray}{0.961} & 0.887/\textcolor{lightgray}{0.980} & 0.730/\textcolor{lightgray}{0.994} & 0.965/\textcolor{lightgray}{0.966} & 0.972/\textcolor{lightgray}{0.970} & \textbf{0.986}/\textcolor{lightgray}{0.977} \\ \bottomrule\bottomrule
    \end{tabular}
}
\label{tab-mint-mvtec}
\end{table*}

\section{Experiments}
\subsection{Datasets and Metrics}
\textbf{Datasets}. We expand on previous research by conducting experiments on a wider range of sensory datasets, including the commonly used MVTec AD~\cite{bergmann2019mvtec} and the newly proposed VisA~\cite{zou2022spot} and BTAD~\cite{mishra2021vt}. The separated setting and unified setting are following existing papers~\cite{you2022unified,Zhao_2023_CVPR,Lu2023HierarchicalVQ}. By testing these datasets, we demonstrate the effectiveness and robustness of the proposed method in detecting anomalies in various industrial settings.
Besides, we use CIFAR-10 to test the performance of semantic AD~\cite{lee2023selformaly}.

% \textbf{MVTec AD Datasets} is a widely used dataset for industrial image anomaly detection, consisting of 15 object categories that can be divided into object images and texture images. It contains a total of 1725 normal and abnormal images, with an additional 3629 normal images used for training. The resolution of each image ranges from 700x700 to 1024x1024 pixels.

% \textbf{VisA Datasets} is currently the largest real-world industrial image anomaly detection dataset with pixel-level labels. It consists of 10,821 images, including 9,621 normal samples and 1,200 abnormal samples, divided into twelve subgroups, each representing a different object. The images are further categorized into single-instance images, multi-instance images, and images with complex structures. The multi-instance images contain multiple objects, while the complex structure images contain a structure or texture-rich object, making VisA more challenging than other datasets.

% TODO: AUPR的重要性
\noindent\textbf{Evaluation Metrics}.
We calculate each category's image-level AUROC (I-AUROC) and report the average of 3 runs. In addition, to better demonstrate the anomaly localization ability of each method~\cite{zou2022spot, xie2023iad}, we use pixel-level AUPR (P-AUPR) to measure the localization performance, which focuses more on the abnormal regions. 
AUPR is also referred to as AP and primarily focuses on the performance of positive classes. 
% It is a more effective metric in situations with class imbalance at the pixel level. 
Several studies, such as spot-diff~\cite{zou2022spot}, have highlighted the influence of different metrics and why AUPR is considered a more informative choice in pixel-wise anomaly detection.
% Unless otherwise specified, the metrics for the following experiments are I-AUROC/P-AUPR. 
% To ensure a fair comparison, we included several state-of-art methods as baselines for comparison. To further improve the comparison, we also trained a unified SimpleNet model on all categories, which is considered the simplest and most effective algorithm currently available.
% separate methods, namely PaDiM~\cite{defard2021padim}, CutPaste~\cite{li2021cutpaste}, PatchCore~\cite{li2022towards}, and SimpleNet~\cite{liu2023simplenet}, as well as the unified model UniAD~\cite{you2022unified}, 
% \paragraph{Implementation Details.}

\noindent\textbf{Implementation Details.}
This section describes the configuration implementation details of the experiments in this paper. 
% As in SimpleNet, PaDiM, and PatchCore, we use a preprocess in that images are resized and center cropped to $256\times256$ and $224 \times 224$, respectively. 
% The extracted feature map size is set to $14\times14$. 
% In this paper, we use the feature maps from the first to the fourth stages of EfficientNet-b4, resize them, and concatenate them together to form a 272-channel feature map. 
The feature maps are extracted from the first to the fourth stages of EfficientNet-b4 (pre-trained in ImageNet). The extracted image feature map size is set to $14\times14$. 
We use the AdamW optimizer with weight decay of $1\times10^{-4}$. All other parts are trained from random initialization except for the pre-trained feature extractor. The model is trained for 1000 full epochs with a batch size of 8 samples on 1 GPU (NVIDIA Tesla V100 32GB). 
The initial learning rate is set to $1\times10^{-4}$ and is decreased by a factor of 0.1 after 800 full epochs. 
% The number of layers in both the encoder and decoder is 6.

% 补充可视化结果
\begin{figure*}[htb]
    \centering
    \includegraphics[width=0.075\textwidth]{NeurIPS/figures/visa_viz/cashew.pdf}
    \includegraphics[width=0.075\textwidth]{NeurIPS/figures/visa_viz/chewinggum.pdf}
    \includegraphics[width=0.075\textwidth]{NeurIPS/figures/visa_viz/fryum.pdf}
    \includegraphics[width=0.075\textwidth]{NeurIPS/figures/visa_viz/pipe_fryum.pdf}
    \includegraphics[width=0.075\textwidth]{NeurIPS/figures/visa_viz/candle.pdf}
    \includegraphics[width=0.075\textwidth]{NeurIPS/figures/visa_viz/capsule.pdf}
    \includegraphics[width=0.075\textwidth]{NeurIPS/figures/visa_viz/macaroni1.pdf}
    \includegraphics[width=0.075\textwidth]{NeurIPS/figures/visa_viz/macaroni2.pdf}
    \includegraphics[width=0.075\textwidth]{NeurIPS/figures/visa_viz/pcb1.pdf}
    \includegraphics[width=0.075\textwidth]{NeurIPS/figures/visa_viz/pcb2.pdf}
    \includegraphics[width=0.075\textwidth]{NeurIPS/figures/visa_viz/pcb3.pdf}
    \includegraphics[width=0.075\textwidth]{NeurIPS/figures/visa_viz/pcb4.pdf}
    \caption{Qualitative results, where sampled image, ground truth, and anomaly map are shown for each class in VisA.}
    \label{visa_figure}
\end{figure*}


% 待修改形式，参考omniAL
\begin{table*}[ht]
\setlength\tabcolsep{3pt}
\centering
\caption{Anomaly detection and localization performance on VisA dataset. We further highlight the best unified-training method in bold. (Metrics: I-AUROC/P-AUPR)}
\label{tab-mint-VisA-image}
\resizebox{0.9\textwidth}{!}{
\begin{tabular}{ll|cccc|ccc}
\toprule\toprule
\multicolumn{2}{c|}{Methods}     & \multicolumn{4}{c|}{Separate}  & \multicolumn{3}{c}{Unified}        \\\midrule
\multicolumn{2}{c|}{Categories}  & PaDiM~\cite{defard2021padim}   & CutPaste~\cite{li2021cutpaste} & PatchCore~\cite{li2022towards} &SimpleNet~\cite{liu2023simplenet} & SimpleNet~\cite{liu2023simplenet} & UniAD~\cite{you2022unified}          & MINT-AD(ours)     \\\midrule
\multirow{4}{*}{\rotatebox{90}{Single}} 
& Cashew      & 0.930/0.522     & 0.848/-     & 0.973/0.585    & 0.980/0.603 & 0.922/\textbf{0.520}&\textbf{0.928}/0.502 & 0.882/0.286 \\
& Chewing gum & 0.988/0.563     & 0.926/-     & 0.991/0.428    &0.998/0.183  &0.959/0.357 &0.996/0.604          & \textbf{0.999}/\textbf{0.624} \\
& Fryum       & 0.886/0.433     & 0.940/-     & 0.962/0.372    &0.987/0.367 &0.913/0.349 &0.898/\textbf{0.476}          & \textbf{0.954}/0.387 \\
& Pipe fryum  & 0.970/0.633     & 0.769/-     & 0.998/0.585    &0.998/0.591 &0.803/\textbf{0.628} &0.978/0.549          & \textbf{0.982}/0.471 \\
                      \midrule
                      \multirow{4}{*}{\rotatebox{90}{Multiple}}

& Candles     & 0.916/0.176     & 0.699/-     & 0.986/0.176    &0.985/0.141 &0.959/0.078 & 0.969/0.212          & \textbf{0.975}/\textbf{0.278} \\
& Capsules    & 0.707/0.182     & 0.790/-     & 0.816/0.687    &0.909/0.577 &0.731/0.442 &0.721/0.513          & \textbf{0.899}/\textbf{0.579} \\
& Macaroni1   & 0.870/0.107     & 0.934/-     & 0.975/0.076   &0.995/0.074  &0.914/0.044 & 0.918/0.088          & \textbf{0.991}/\textbf{0.240} \\
& Macaroni2   & 0.705/0.011     & 0.836/-     & 0.781/0.035    &0.823/0.049 &0.604/0.010 &0.856/0.039          & \textbf{0.901}/\textbf{0.158} \\
                      \midrule
                      \multirow{4}{*}{\rotatebox{90}{Complex}}

& PCB1        & 0.947/0.519     & 0.831/-     & 0.985/0.917    &0.996/0.849 &0.910/\textbf{0.943} &0.957/0.674          & \textbf{0.965}/0.782 \\
& PCB2        & 0.885/0.138     & 0.449/-     & 0.973/0.143   &0.995/0.131  &0.915/0.148 &0.934/0.089          & \textbf{0.964}/\textbf{0.277} \\
& PCB3        & 0.910/0.288     & 0.900/-     & 0.979/0.389    &0.992/0.442 &0.889/0.303 &0.894/0.149          & \textbf{0.980}/\textbf{0.340} \\
& PCB4        & 0.975/0.184     & 0.907/-     & 0.996/0.424    &0.995/0.378 &0.961/0.331 &\textbf{0.994}/\textbf{0.365}          & 0.988/0.304 \\
                      \midrule
& {\textbf{Mean}}         & 0.891/0.309  & 0.819/- & 0.951/0.401     &0.971/0.365 &0.873/0.338 &0.920/0.355     & \textbf{0.957}/\textbf{0.394}\\
\bottomrule\bottomrule

\end{tabular}}
\end{table*}

\subsection{Anomaly Detection and Localization on MVTec-AD}
The results of anomaly detection on the MVTec-AD dataset are presented in Table~\ref{tab-mint-mvtec}. 
In the unified setting, although UniAD~\cite{you2022unified} and OmniAL~\cite{Zhao_2023_CVPR} are both unified reconstruction networks, MINT-AD significantly improves the performance of most categories. What's more, MINT-AD demonstrates even more significant advantages for categories that can be further subdivided, such as Toothbrush, Capsule, and Screw. This indicates that our proposed algorithm can reduce interference in both inter-class and intra-class and has better normal reconstruction ability from a classification perspective. 
While the performance of the separate methods is still inferior to that of the current best separate method, our proposed method significantly outperforms the Synthesizing-based method CutPaste~\cite{li2021cutpaste} and the Ensembling-based method PaDiM~\cite{defard2021padim}. It is worth noting that the SOTA separate method, SimpleNet, performs poorly with unified training because SimpleNet uses a discriminator model, and simply fusing multi-class information together for training would result in a significant drop in performance. In contrast, our proposed method, MINT, performed best under the unified framework. To further demonstrate the effectiveness of our proposed method, we visualize representative samples for anomaly localization using MINT-AD in Figure \ref{mvtec_figure}.

\subsection{Anomaly Detection and Localization on VisA} 
In order to conduct a more comprehensive analysis, we opted for the VisA~\cite{zou2022spot} dataset, which also incorporates categories with multiple instances and complex structures, going beyond simple single-instance anomaly detection. 
% Table ~\ref{tab-mint-VisA-image} revealed that almost all methods experienced a certain degree of decline in performance, with PaDiM~\cite{defard2021padim} exhibiting a decrease of approximately 0.1 in the P-AUPR metric. This decline in performance may be attributed to the fact that the defects in the VisA dataset are smaller and finer, some of which are located at the edges. 
Upon analyzing the results in Table~\ref{tab-mint-VisA-image}, MINT-AD achieves a larger improvement than UniAD in the unified setting in VisA compared with MVTec AD. By comparing the I-AUROC and P-AUPR metrics for each category, we found that the advantage of MINT-AD mainly stems from its more balanced performance across all categories. This implies a reduction in `` inter-class interference''. 
In the separate setting, we found that SimpleNet~\cite{liu2023simplenet} still achieved SOTA performance in I-AUROC. Despite training with multi-class, our method has just a slightly lower I-AUROC than separate SimpleNet, but a higher P-AUPR. 
Additionally, we observed that for some non-rigid objects, such as Macaroni, the P-AUPR of all methods was very low due to the shape of the object changing to some extent. 
% This made it difficult to generalize even with limited data training using methods such as reconstruction, embedding, or synthesizing. 
% Furthermore, SimpleNet trained under the unified framework showed less decline in performance on the VisA dataset than on the MVTec dataset, possibly because there are fewer categories in VisA, and the similarity between categories is relatively high. 
Overall, our method demonstrated better adaptability to complex scenes and achieved the best performance in the unified methods. Some qualitative results are shown in Figure~\ref{visa_figure}. 

% In the experiments on the VisA dataset, the simplenet algorithm and the memory-based PatchCore, which were proposed together with the dataset, were also compared. The powerful performance of PatchCore has been explained in the previous chapter, while MINT-AD increases the feature resolution to 28*28, which on the one hand increases the difficulty of the reconstruction model, and on the other hand is more conducive to fine segmentation.

% As shown in Table~\ref{tab-mint-VisA-image}, on the larger VisA dataset, the advantage of MINT-AD in anomaly detection is more significant compared to UniAD, with an average error reduction of 0.25. Especially for multi-instance categories with more complex distributions and categories with complex structures, MINT-AD has a greater improvement over UniAD due to its better distribution robustness. In this dataset, the performance of MINT-AD is closer to that of separately trained PatchCore. Specifically, UniAD has an advantage in simple instance categories, while MINT-AD performs better in multi-instance categories and categories with complex structures.



% 补充可视化结果

% \subsection{Anomaly detection and localization on BATD}
% As for the results on the BTAD dataset shown in Table~\ref{tab-mint-btad}, since the number of categories is only three, much smaller than the other two datasets, MINT's ability to resist interference from multiple categories is not so prominent.

% \begin{table}[ht]
% % \small
% \centering
% \caption{The anomaly detection and localization performance on BTAD, with AUROC used as the detection metric and AUPR used as the localization metric.}
% \label{tab-mint-btad}
% \begin{tabular}{lcccc}
% \toprule
% Metrics       & \multicolumn{2}{c}{Detection}  & \multicolumn{2}{c}{localization} \\\midrule
% \textbf{Categories} & UniAD    & MINT(ours)  & UniAD    & MINT(ours)   \\\midrule
% 01                & \textbf{0.998} & 0.996 & \textbf{0.520}& 0.518 \\
% 02                & 0.782          & \textbf{0.785} & 0.335      & \textbf{0.407} \\
% 03                & \textbf{0.999} & \textbf{0.999} & 0.573      & \textbf{0.587} \\\midrule
% Mean              & 0.926          & \textbf{0.927} & 0.476      & \textbf{0.504} \\\bottomrule
% \end{tabular}
% \end{table}

% TODO: more detail
\subsection{Performance in Larger Dataset}
\label{larger-dataset}
% From Table \ref{tab-mint-mvtec-image} and Table \ref{tab-mint-VisA-image}, it can be seen that SimpleNet is greatly affected by the number of categories, and it performs better in situations where there are fewer categories or when the inter-class variation is low (e.g., VisA) compared to MVTec. 
To explore how the unified models perform with an increased number of categories, we conducted training using a larger merged dataset consisting of the MVTec, VisA, and BTAD anomaly detection datasets. The corresponding results are presented in Table~\ref{tab-mint-all}, where the superiority of MINT-AD over UniAD becomes more evident. Specifically, when faced with the pressure of unexpected multi-class scenarios, our method still experiences certain performance degradation, with a decrease of 0.018 in I-AUROC on MVTec AD and a decrease of 0.033 on VisA. This may be due to the limited ability of the reconstruction model to fit fine-grained feature details. UniAD uses an equal-sized base reconstruction model but performs worse. This demonstrates that our class-aware network has better robustness when the number of classes increases. 

\begin{table}[hbt]
    \centering
    \caption{Performance comparison of algorithms on a unified Dataset Comprising MVTec, VisA, and BTAD where 30 categories are combined for unified training. (I-AUROC/P-AUPR)}
    \label{tab-mint-all}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{l|ccc|c}
    \toprule\toprule
        Methods & BTAD~\cite{mishra2021vt} & MVTec~\cite{bergmann2019mvtec} & VisA~\cite{zou2022spot} & Mean \\ \midrule
        UniAD & 0.921/\textbf{0.469}  & 0.936/0.416  & 0.906/0.336  & 0.923/0.389  \\ 
        MINT-AD & \textbf{0.954}/0.445  & \textbf{0.969}/\textbf{0.450 }  & \textbf{0.924}/\textbf{0.359}  & \textbf{0.949}/\textbf{0.413} \\ \bottomrule\bottomrule
    % Methods & BTAD~\cite{mishra2021vt} & MVTec~\cite{bergmann2019mvtec} & VisA~\cite{zou2022spot} & Mean \\ \midrule
    % UniAD & 92.1/\textbf{46.9}   & 93.6/41.6   & 90.6/33.6   & 92.3/38.9   \\ 
    % MINT-AD & \textbf{95.4}/44.5   & \textbf{96.9}/\textbf{45.0}   & \textbf{92.4}/\textbf{35.9}   & \textbf{94.9}/\textbf{41.3}  \\ \bottomrule
    \end{tabular}}
\end{table}

\begin{table}[ht]
% \setlength\tabcolsep{2pt}
\caption{Anomaly detection results with AUROC metric on CIFAR-10 under the unified case. Here, \{01234\} means samples from classes 0, 1, 2, 3, and 4 are borrowed as the normal ones.}
\label{tab-cifar10}
\resizebox{\linewidth}{!}{
\begin{tabular}{c|cccccc|c}
\toprule\toprule
Normal Indices & US & FCDD  & FCDD+OE  & PANDA  & MKD  & UniAD  & MINT-AD \\
\midrule$\{01234\}$ & 0.513 & 0.550 & 0.718 & 0.666 & 0.642 & 0.844 & \textbf{0.867} \\
$\{56789\}$ & 0.513 & 0.503 & 0.737 & 0.732 & 0.693 & 0.809 & \textbf{0.833} \\
$\{02468\}$ & 0.639 & 0.592 & 0.853 & 0.771 & 0.764 & 0.930 & \textbf{0.936} \\
$\{13579\}$ & 0.568 & 0.585 & 0.850 & 0.729 & 0.787 & 0.906 & \textbf{0.926} \\
\midrule 
\textbf{Mean} & 0.559 & 0.558 & 0.789 & 0.724 & 0.721 & 0.872 & \textbf{0.891} \\
\bottomrule\bottomrule
\end{tabular}
}
\end{table}

\subsection{Anomaly detection on CIFAR-10}
For semantic anomalies, we make experiments on CIFAR-10. The experiment adopts the settings of UniAD, which consists of four combinations. For each combination, five categories collectively serve as normal samples, while other categories are treated as anomalies. The class indices refer to the class labels. The results are shown in the table \ref{tab-cifar10}, with MINT-AD outperforming other anomaly detection methods. This demonstrates the applicability of our proposed method to global semantic anomalies as well. 
% \clearpage
\subsection{Ablation studies}
% In this paper, ablation experiments were conducted on various modules of MINT-AD on the MVTec dataset, and the experimental results are shown in Table~\ref{tab:mint-ablation}. The results show that increasing feature resolution is effective on this dataset, but in the UniAD experiment, increasing resolution is harmful, which requires further exploration in the future. The addition of classification loss is an important reason for further improving the model's unified learning ability, but even without classification loss, the model's performance is still better than UniAD. This is because the classification network structure itself distinguishes the data, indicating that the reconstruction loss and prior loss also need to model classification when facing multi-class data. We found that the attention mechanism with neighbor masking is not always effective for MINT, which is inconsistent with the conclusion in UniAD. The analysis in this paper suggests that after the model has the ability to distinguish between different categories, reconstruction can rely more on the implicit representation network output query, which avoids the "shortcut" problem in UniAD. Therefore, NMA at this time may reduce the model's reconstruction ability and affect its performance.
% \subsection{Comparison with Class-aware Architectures}
% The figure illustrates our analysis of various class embedding methods, namely label-onehot embedding, multi-query selected embedding, text embedding, and class-aware embedding. It is worth noting that the first three methods require the corresponding class information to be known at test time, whereas class-aware embedding does not rely on such information.

% \begin{table*}[t]
% \begin{minipage}{0.45\textwidth}
% \centering
% \renewcommand\arraystretch{1.0}
% \begin{tabular}{lcc}
% \toprule
% Methods & I-AUROC & P-AUPR \\ \midrule
% No Class Info & 0.975 & 0.445\\
% Label Embedding & 0.979  & 0.470\\
% Multi-query & 0.976  & 0.470\\
% Text query  & 0.977  & 0.463\\
% Class-aware Query  & \textbf{0.986}  & \textbf{0.498} \\ \bottomrule
% \end{tabular}
% \caption{Different class embedding methods.}
% \label{tab:class_embedding}
% \end{minipage}
% \hfill
% \begin{minipage}{0.5\textwidth}
% \centering
% \begin{tabular}{cccccc}
% \toprule
% PreProcess & $L_{CE}$ & $L_{Prior}$& $Q_{Class}$ &I-AUROC & P-AUPR \\
% \midrule
% & & & & 0.975 & 0.445 \\
% \Checkmark& & &   &  0.977  & 0.462\\
% \Checkmark&     \Checkmark&  &   &  0.977  & 0.465\\
% \Checkmark&    \Checkmark  &  & \Checkmark  & 0.981  & 0.477 \\
% \Checkmark& \Checkmark  & \Checkmark  & & 0.983  & \textbf{0.502} \\
% \Checkmark  &\Checkmark  & \Checkmark  & \Checkmark  & \textbf{0.986}  & 0.498  \\
% \bottomrule
% \end{tabular}
% \caption{Different submodule ablation study, \Checkmark represents the use of the corresponding operation.}
% \label{tab:mint-ablation}
% \end{minipage}
% \end{table*}


\begin{table}[ht]
\centering
\caption{Different class-aware methods. \Checkmark represents using labels in training/testing stage.}
\resizebox{\linewidth}{!}{
    \begin{tabular}{lcccc}\\\toprule\toprule
    \multirow{2}{*}{Methods} & \multicolumn{2}{c}{Using Label} & \multirow{2}{*}{I-AUROC} & \multirow{2}{*}{P-AUPR}\\ \cline{2-3} 
    & Training & Testing & & \\
    % \multirow{2}{*}{Method} & \multicolumn{2}{l}{Accuracy} & \multicolumn{2}{l}{Round (GA=)} \\
    %     &        $GA$ & $LA$ & $30\%$ & $40\%$ \\ \hline
    \midrule
    Vanilla UniAD  & - & - & 0.965 & 0.445\\
    with Class Token & \Checkmark & \Checkmark & 0.979  & 0.470\\  
    with Query Pool & \Checkmark & \Checkmark & 0.976  & 0.470\\  
    with Text Prompt  & \Checkmark & \Checkmark & 0.977  & 0.463\\   \midrule 
    \emph{Prompt Type of MINT-AD}&&& \\
    Image Prompt & - & - & 0.978 & 0.465 \\ 
    Label Prompt & \Checkmark & \Checkmark & 0.980 & 0.472 \\ 
    Feature Prompt & \Checkmark & - & \textbf{0.986}  & \textbf{0.498} \\  
    \midrule 
    % Text-encoder & & \\  
    INR $\rightarrow$ MLP & \Checkmark & - & 0.980 & 0.498 \\ 
    \bottomrule\bottomrule
    \end{tabular}
}
   \label{tab:class_embedding}
\end{table}

\noindent\textbf{Class-aware Embedding}. We conducted an investigation into the impact of class embedding methods and developed three class embedding methods based on the previously mentioned methods ~\cite{xu2022multi, dong2022category, xie2023category}. The first block of Table~\ref{tab:class_embedding} was used to compare the performance, while Figure~\ref{fig:class_embed} provided a schematic diagram of methods. We utilized UniAD without class information as the baseline. 
We discovered that directly concatenating class information with input features resulted in improved metrics, indicating the advantage of class information on network performance. While the three class-aware improvements vary significantly, they all effectively utilize the label as a prompt.

\noindent\textbf{Prompt Types.} We further compare the three prompt types mentioned in Figure \ref{fig:MINT}. 
Firstly, we can observe in the second block of Table~\ref{tab:class_embedding} that when using the label as a prompt, our performance is better than the previous three methods, indicating that the INR network we use is superior. Secondly, it can be noticed that using features from the classification network as prompts is the optimal choice because it provides finer-grained classification compared to the label. Using the image as a prompt does not use any label, but it still offers a certain performance improvement compared to UniAD due to the network advantage.  

% However, using multiple queries did not significantly enhance the metrics compared to directly concatenating class information. Additionally, we employed the widely used CLIP~\cite{radford2021learning} model to get text-aware queries. 
% However, P-AUPR decreased compared to the above two methods. This could be attributed to the fact that CLIP was trained on natural scenes but not industry scenes. Our method with class prompt implicit neural representation outperforms other methods and fully demonstrates the effectiveness of our approach. 
\begin{table}[htb]
\centering
\scriptsize
\caption{Different submodule ablation study, \Checkmark represents the use of the corresponding operation.}
\label{tab:mint-ablation}
\small
\resizebox{0.95\linewidth}{!}{
\begin{tabular}{cccccc}
\toprule\toprule
$Adapter$ & $L_{CE}$ & $L_{Prior}$& $Query$ &I-AUROC & P-AUPR \\
\midrule
% & & & & 0.975 & 0.445 \\
% \Checkmark& & &   &  0.977  & 0.462\\
-& -& -& -& 0.971 & 0.447 \\
\Checkmark& - & -&  - &  0.975  & 0.445\\
\Checkmark& \Checkmark &  -& -  &  0.977  & 0.465\\
\Checkmark& \Checkmark  & - & \Checkmark  & 0.981  & 0.477 \\
\Checkmark& \Checkmark  & \Checkmark  & -& 0.983  & \textbf{0.502} \\

% & \Checkmark  & \Checkmark  &       &\Checkmark& 0.932  & 0.353   \\
% \Checkmark& \Checkmark  & \Checkmark  &  \Checkmark && 0.875  & 0.316   \\
\Checkmark  &\Checkmark  & \Checkmark  & \Checkmark  & \textbf{0.986}  & 0.498  \\
\bottomrule\bottomrule
\end{tabular}
}
\end{table} 

\noindent\textbf{Architecture Design}. The last block of Table~\ref{tab:class_embedding} shows the performance when replacing the INR network with a large MLP. Despite having over 500 times more parameters than INR, MLP still struggles to achieve the mapping capability of INR.
Table~\ref{tab:mint-ablation} presented below displays the outcomes of ablation experiments conducted on each key operation of MINT-AD, including the adapter, the classification loss, the prior loss, and the class-aware embedding query. The results show that the feature adapter is useful for detection. It was observed that the classification loss had a negligible impact on performance. Further analysis of the impact of prior loss and class-aware embedding query revealed that both contributed to the improvement in performance. However, the inclusion of prior loss significantly enhanced pixel-level metrics by computing the mean and variance of the pixel distribution for the corresponding class, thereby aligning the reconstruction results with the distribution. Finally, combining all modules significantly improved image-level metrics, while pixel-level metrics slightly decreased compared to not using query embedding. This could be attributed to the class query focusing more on global class information, which may have a negative impact on pixel-level metrics. 

% The results show that image preprocessing enhances pixel-level metrics by approximately two points, which could be attributed to the object occupying a larger proportion of the image, thereby reducing false positives in the background. 



% TODO: 补充相关模型的FLOPS, Learnable Params(M)和耗时，其中Separate要*相对应的类别
% \subsection{Inference Time and Complexity Analysis}
% Although our method is a unified approach, the corresponding computational complexity and inference time have not increased. On the contrary, compared with methods such as storing feature embeddings in memory, our method has lower memory requirements, as shown in the table.
% \begin{table}[]
% \centering
% \begin{tabular}{llllllll}
% \toprule
%                 & PaDiM & DRAEM & cutpaste & patchcore & simpleness & UniAD & Ours \\ \midrule
% FLOPS           &       &       &   &           &            &       &      \\
% Memory Usage    &       &       &   &           &            &       &      \\
% Inference times &       &       &   &           &            &       &     \\ \bottomrule
% \end{tabular}
% \end{table}

% TODO: 补充可视化结果，包括异常检测的可视化和加入class embedding后重建特征对应T-sne的可视化。
% \subsection{Qualitative Results}
% We demonstrate the comparison between MINT-AD and current state-of-the-art methods on the MVTec and VisA datasets. In Figure 3, we can observe that the features become more clustered after class embedding, and compared with other methods, although we are a unified model, our localization and detection performance are better on certain categories.


==> CVPR/sec/5_conclusion.tex <==
\section{Conclusion}
We investigate multi-class anomaly detection scenarios and propose a category-aware unified reconstruction network. It innovatively applies implicit neural representation in anomaly detection, mapping category encoding to feature space. To address the fitting of multiple samples within the same class, our model learns the category distribution by predicting the prior distribution and proposes a prior loss to update the network. Experimental results show that this paper's proposed MINT-AD algorithm outperforms existing algorithms on multiple datasets.

\noindent \textbf{Discussion.} In this work, we did not establish connections with relevant classes in anomaly detection. We believe that this is a reasonable direction for future improvements. At the same time, the security of the data and labels has not been fully studied. When applied in monitoring, it may be vulnerable to backdoor attacks, leading to privacy leaks. 

% In the future, researchers can try to find the relationships between different categories, which may further improve performance and reduce costs. 
% If the features of multiple categories can be correlated, the network capacity can be reduced to lower computational costs. 
% At the same time, the security of the anomaly detection model has not been fully studied. When applied in monitoring and other fields, it may be vulnerable to backdoor attacks, leading to privacy leaks.
